STrack: A Reliable Multipath Transport for AI/ML Clusters

Emerging artificial intelligence (AI) and machine learning (ML) workloads present new challenges of managing the collective communication used in distributed training across hundreds or even thousands of GPUs. This paper presents STrack, a novel hardware-offloaded reliable transport protocol aimed at improving the performance of AI /ML workloads by rethinking key aspects of the transport layer. STrack optimizes congestion control and load balancing in tandem: it incorporates an adaptive load balancing algorithm leveraging ECN, while adopts RTT as multi-bit congestion indicators for precise congestion window adjustment. Additionally, STrack facilitates out-of-order delivery, selective retransmission, and swift loss recovery in hardware for multipath environment. The extensive simulation comparing STrack and RoCEv2 demonstrates that STrack outperforms RoCEv2 by up to 6X with synthetic workloads and by 27.4% with collective workloads, even with the optimized RoCEv2 system setup.

==> Makefile <==
#
# $Id: Makefile,v 1.1 2006/06/27 21:10:04 shafer Exp $
#
# Makefile for converting tex files to PDF
#

PAPER = main

# directories
OUTPUT_DIR = ./
BIB_OUT_FILE = bib-issues

# paths
BIB_PATH="$(TEXT_DIR)"
BST_PATH="$(STYLE_DIR):$(shell kpsewhich --progname=latex --show-path=.bst)"
TEX_PATH="$(TEXT_DIR):$(STYLE_DIR):$(STYLE_DIR)/sty:$(shell kpsewhich -progname=tex -show-path=tex)"

# options
BIBTEX_OPTS = -terse
DVIPS_OPTS = -q -G0 -tletter
LATEX_OPTS  = -output-directory=$(OUTPUT_DIR) -file-line-error -interaction=batchmode
MAKEINDEX_OPTS = -q
PS2PDF_OPTS = -q -sPAPERSIZE=letter -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress \
              -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true

#commands
LATEXC = max_print_line=1000 pdflatex
PRINT_LATEX_ERRORS = (cat $(PAPER).log | grep '^[^: ]*:[^: ]*:' || exit 0)
PRINT_LATEX_WARNINGS = (cat $(PAPER).log | grep -i 'latex warning' || exit 0)
PRINT_BIBTEX_WARNINGS = (cat *.blg | grep '^Warning' | sort | uniq > $(BIB_OUT_FILE) || exit 0)
PRINT_BIBTEX_NOTE = if [ -s $(BIB_OUT_FILE) ]; then \
                    echo "$(NOTE_LABEL)Bibliography warnings written to '$(BIB_OUT_FILE)'."; fi


all: $(PAPER).pdf

#
# We want our main "pdf" to depend on all the "tex" and "bib" source
#

#main.pdf: sig-alternate-10pt.cls *.tex *.bib figures/*
#main.pdf: acmart.cls *.tex *.bib figures/*

main.pdf: *.tex *.bib  
#
# Now provide the rules for building the various targets and
# intermediate targets
#

%.pdf : %.tex
	@echo "$(LATEX_LABEL)Performing initial latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

	@echo "$(BIBTEX_LABEL)Processing bibliography..."
	@BIBINPUTS=$(BIB_PATH) \
	 BSTINPUTS=$(BST_PATH) \
		bibtex $(BIBTEX_OPTS) $(PAPER) | grep -v "^Warning"; \
		if [ $${PIPESTATUS[0]} != 0 ]; then \
			rm -f $@ && exit 1; \
		fi
	@-$(PRINT_BIBTEX_WARNINGS)
	@-$(PRINT_BIBTEX_NOTE)


	@echo "$(LATEX_LABEL)Performing secondary latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)


	@echo "$(LATEX_LABEL)Performing final latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)
	@-$(PRINT_LATEX_WARNINGS)


%.ps : %.dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -j0 -o $@ $<

# %.pdf : %.ps
# 	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true -dCompatibilityLevel=1.2 -dProcessColorModel=/DeviceGray -dSubsetFonts=true -dMaxSubsetPct=100 $< $@

clean:
	-rm -f *.dvi *.log *.aux *.bbl *.blg *.ent *.out main.pdf

#
# Run "make balance" after adding balance columns at the right place
#

balance:
	latex main
	latex main
	dvips -o main.ps main.dvi
	ps2pdf main.ps main.pdf

